Discourse-Aware Neural Extractive Text Summarization

Recently BERT has been adopted for document encoding in state-of-the-art text summarization models. However, sentence-based extractive models often result in redundant or uninformative phrases in the extracted summaries. Also, long-range dependencies throughout a document are not well captured by BERT, which is pre-trained on sentence pairs instead of documents. To address these issues, we present a discourse-aware neural summarization model - DiscoBert. DiscoBert extracts sub-sentential discourse units (instead of sentences) as candidates for extractive selection on a finer granularity. To capture the long-range dependencies among discourse units, structural discourse graphs are constructed based on RST trees and coreference mentions, encoded with Graph Convolutional Networks. Experiments show that the proposed model outperforms state-of-the-art methods by a significant margin on popular summarization benchmarks compared to other BERT-base models.

==> fig_graph_vis.tex <==
% [width=0.48125\textwidth] for ACL
% [width=0.473\textwidth] for AAAI
\begin{figure}[t]
\centering
% \justify
\small
% {Example: [Police]\textsubscript{1} [investigating the case]\textsubscript{2}  [learned]\textsubscript{3}  [where 36-year-old Vittorio Arrigoni was being held]\textsubscript{4}  [and went to the location,]\textsubscript{5}  [where they found the body,]\textsubscript{6}  [the statement said.]\textsubscript{7} }
\includegraphics[width=0.48\textwidth]{graph_example.pdf}
\caption{Examples of the adjacent matrix of Coreference Graph $\mathcal{G}_{C}$ and RST Graph $\mathcal{G}_{R}$. 
}
\label{fig:vis}
\end{figure}
% Police investigating the case learned where 36-year-old Vittorio Arrigoni was being held and went to the location, where they found the body, the statement said.

==> tab_coref_example.tex <==
% [width=0.48125\textwidth] for ACL
% [width=0.473\textwidth] for AAAI

% Police investigating the case learned where 36-year-old Vittorio Arrigoni was being held and went to the location, where they found the body, the statement said.


% \textquote{ [ The Financial Accounting Standards Board 's coming rule on disclosure] \textsubscript{1} $\cdots$ }
\definecolor{darkgrey}{HTML}{579d42}
\definecolor{lightgrey}{HTML}{D5D5D5}
\definecolor{strongorange}{HTML}{DF9945}

 \begin{quote}
 \small
 [\colorbox{darkgrey}{\color{white}The Financial Accounting Standards Board}'s coming rule on disclosure]\textsubscript{1} $\cdots$ [\colorbox{darkgrey}{\color{white}FASB} is proposing another accouting delay.]\textsubscript{5} $\cdots$ [\colorbox{darkgrey}{\color{white}FASB}’s proposed \colorbox{lightgrey}{CECL} delay would affect only smaller reporting companies.]\textsubscript{9} [said \colorbox{darkgrey}{\color{white}FASB} Chairman \colorbox{strongorange}{\color{white}Russ Golden}.]\textsubscript{21} $\cdots$ [\colorbox{strongorange}{\color{white}he} said in a statement.]\textsubscript{24} $\cdots$
 \end{quote}
 
